Surrogate Losses for Online Learning of Stepsizes in Stochastic Non-Convex Optimization

Stochastic Gradient Descent (SGD) has played a central role in machine learning. However, it requires a carefully hand-picked stepsize for fast convergence, which is notoriously tedious and time-consuming to tune. Over the last several years, a plethora of adaptive gradient-based algorithms have emerged to ameliorate this problem. They have proved efficient in reducing the labor of tuning in practice, but many of them lack theoretic guarantees even in the convex setting. In this paper, we propose new surrogate losses to cast the problem of learning the optimal stepsizes for the stochastic optimization of a non-convex smooth objective function onto an online convex optimization problem. This allows the use of no-regret online algorithms to compute optimal stepsizes on the fly. In turn, this results in a SGD algorithm with self-tuned stepsizes that guarantees convergence rates that are automatically adaptive to the level of noise.

==> 2stepsizes.tex <==
\section{Adapting Two or More Stepsizes}

In this section, we show another application of our surrogate losses, to adapt two update strategies at the same time.

Consider the classic SGD with momentum~\cite{Polyak64}, where we update with
\begin{align*}
\bz_{t+1} &= \alpha_t \bz_t + G(\bx_t,\xi_t) \\
\bx_{t+1} &= \bx_t - \eta_t \bz_{t+1}~.
\end{align*}
The above the be equivalently written as 
\begin{align*}
\bx_{t+1}=\bx_t - \eta_t G(\bx_t,\xi_t) - \beta_t \bz_t,
\end{align*}
where $\beta_t=\alpha_t \eta_t$. In words, the momentum update corresponds to a standard update using the negative stochastic gradient $G(\bx_t,\xi_t)$ with stepsize $\eta_t$, augmented by another update in the direction of $-\bz_t$ and stepsize $\beta_t$. When the noise is zero, we know that a properly tuned momentum term can give us an accelerated rate~\cite{Polyak64}. However, in the presence of noise the acceleration is destroyed and a plain SGD would be preferable, i.e. setting $\beta_t$ to zero.
This immediately inspires us to extend the use of surrogate losses to tune multiple stepsizes for different updates: we can use the surrogate losses to automatically set both the stepsizes of $\eta_t$ and $\beta_t$. Using a no-regret online learning algorithm, we will be guaranteed to be as good as any fixed setting of $\eta_t$ and $\beta_t$. This means that the resulting algorithm will have a convergence rate that is never much worse than the one of plain SGD, and could be much better in the case that the momentum term is useful.

Note that the framework is general enough to support any finite number of updates, but, for the sake of clarity, we will state the algorithm and result only for one additional update beyound the one using $G(\bx_t,\xi_t)$.

Define the surrogate losses as
\begin{align*}
\ell^\eta_t(\eta) &=-\langle \eta G(\bx_t,\xi_t), G(\bx_t,\xi'_t) \rangle + M \eta^2 \|G(\bx_t,\xi_t)\|^2, \\
\ell^\beta_t(\beta) &=-\langle \beta \bz_t, G(\bx_t,\xi'_t) \rangle + M \beta^2 \|\bz_t\|^2,
\end{align*}
where $G(\bx_t,\xi_t)$ and $G(\bx_t,\xi'_t)$ are the noisy stochastic gradients received from the black-box oracle at time $t$.
Define also the following regrets
\begin{align*}
\mathrm{Regret}^\eta_T(\eta) &=\sum_{t=1}^T (\ell_t^\eta(\eta_t)- \ell_t^\eta(\eta))\\
\mathrm{Regret}^\beta_T(\beta) &=\sum_{t=1}^T (\ell_t^\beta(\beta_t)- \ell_t^\beta(\beta))~.
\end{align*}

Analogously to Theorems~\ref{thm:surrogate} and Theorem~\ref{thm:olsmooth}, we have the following theorems.
\begin{thm}
\label{thm:surrogate_two_vars}
Assume \textbf{H4} to hold and $\eta_t$ and $\beta_t$ to be independent from $\xi_j$ and $\xi'_j$ for $j\geq t$. Then,
\[
\E\left[f(\bx_{t+1})-f(\bx_t)\right]
\leq \E\left[\ell^\eta_t(\eta_t)+\ell_t^\beta(\beta_t)\right]~.
\]
\end{thm}

\begin{thm}
\label{thm:olsmooth_two_vars}
Assume \textbf{(H1, H2, H4)} to hold. Then, for any $\eta>0$, Algorithm~\ref{algo:sgdol} satisfies
\begin{align*}
\E&\left[\left(\eta-\frac{M}{2}\eta^2\right)\sum_{t=1}^T \|\nabla f(\bx_t)\|^2\right] \\
&\leq f(\bx_1) - f^\star + \E\left[\mathrm{Regret}^\eta_T(\eta)+\mathrm{Regret}^\beta_T(0)\right] \\
&\quad + M \eta^2\sum^T_{t=1} \E[\sigma_t^2]~.
\end{align*}
\end{thm}

Note that in the above theorems we do not assume anything on the update direction $\bz_t$.

% \begin{thm}
% Let $\lambda>0$ and set $\eta_0=\frac{4}{(\sqrt{M}+\sqrt{\lambda})^2}$, $\beta_0=\frac{\sqrt{M}-\sqrt{\lambda}}{\sqrt{M}+\sqrt{\lambda}}$, and $\bz_t=\bx_t-\bx_{t-1}$
% Assume $\textbf{H1-H4}$ hold. Then SGDOL$^2$ in Algorithm~\ref{} satisfies
% \[
% \E_i[\|\nabla f(\bx_i)\|^2]
% \leq O\left(\frac{f(\bx_1)-f^\star}{T}+\frac{\sigma}{\sqrt{T}}\right)~.
% \]
% In addition, if the function is $m$-strongly convex, where $m\geq\lambda$, and $\sigma^2=0$, we have
% \[
% \|\bx_{T+1} - \bx^\star\|
% \leq \left( \frac{\sqrt{\kappa}-1}{\sqrt{\kappa}+1}\right)^T \|\bx_1 - \bx^\star\|~.
% \]
% \end{thm}
%
% \begin{proof}
% The proof of the first part follows from Theorem~\ref{thm:olsmooth_two_vars}. For the second part, observe that if $\sigma=0$,
% \end{proof}

